Solving ImageNet: a Unified Scheme for Training any Backbone to Top Results

ImageNet serves as the primary dataset for evaluating the quality of computer-vision models. The common practice today is training each architecture with a tailor-made scheme, designed and tuned by an expert. In this paper, we present a unified scheme for training any backbone on ImageNet. The scheme, named USI (Unified Scheme for ImageNet), is based on knowledge distillation and modern tricks. It requires no adjustments or hyper-parameters tuning between different models, and is efficient in terms of training times. We test USI on a wide variety of architectures, including CNNs, Transformers, Mobile-oriented and MLP-only. On all models tested, USI outperforms previous state-of-the-art results. Hence, we are able to transform training on ImageNet from an expert-oriented task to an automatic seamless routine. Since USI accepts any backbone and trains it to top results, it also enables to perform methodical comparisons, and identify the most efficient backbones along the speed-accuracy Pareto curve. Implementation is available at:https://github.com/Alibaba-MIIL/Solving_ImageNet

==> Conclusion.tex <==
In this paper, we present an asymmetric loss (ASL) for multi-label classification.
% We identified the issues in other well-known symmetric loss criteria, such  as cross-entropy and focal loss, that are being used for multi-label classification problems. 
ASL contains two complementary asymmetric mechanisms, which
operate differently on positive and negative samples. By examining ASL derivatives, we gained a deeper understanding of the loss properties. Through network probability analysis, we demonstrate the effectiveness of ASL in balancing between negative and positive samples, and proposed an adaptive scheme that can dynamically adjusts
the asymmetry levels throughout the training. Extensive experimental analysis shows that ASL outperforms common loss function and previous state-of-the-art approaches 
on popular multi-label classification benchmarks, including MS-COCO, Pascal-VOC, NUS-WIDE and Open Images.
% We also tested ASL on object detection and fine-grain single-label classification datasets,
% demonstrating its applicability to other computer vision tasks that also exhibit  dataset imbalancing. 


==> Tables/aug_repeats.tex <==
\begin{table}[hbt!]
\centering

\begin{tabular}{c|c} 
\Xhline{3\arrayrulewidth}

Aug Repeats    & Top1 Acc. [\%]  \\ 
\Xhline{3\arrayrulewidth}
1 (no repeats) & TBD             \\
2              & TBD             \\
3              & TBD          \\
\hline
\end{tabular}
\caption{TBD}
\label{Table:aug_repeats}
\end{table}
